A Study of Muon Neutrino Disappearance Using the Fermilab Main Injector Neutrino Beam

We report the results of a search for muon-neutrino disappearance by the Main Injector Neutrino Oscillation Search. The experiment uses two detectors separated by 734 km to observe a beam of neutrinos created by the Neutrinos at the Main Injector facility at Fermi National Accelerator Laboratory. The data were collected in the first 282 days of beam operations and correspond to an exposure of 1.27e20 protons on target. Based on measurements in the Near Detector, in the absence of neutrino oscillations we expected 336 +/- 14 muon-neutrino charged-current interactions at the Far Detector but observed 215. This deficit of events corresponds to a significance of 5.2 standard deviations. The deficit is energy dependent and is consistent with two-flavor neutrino oscillations according to delta m-squared = 2.74e-3 +0.44/-0.26e-3 eV^2 and sin^2(2 theta) > 0.87 at 68% confidence level.

==> data_mc.tex <==
\pstart
The large data samples collected in the Near Detector for various beam configurations ($2.6\times10^{6}$ events in the fiducial region for the LE010/185kA configuration) allowed detailed comparisons with Monte Carlo to be carried out. These comparisons enabled us to verify our detector simulation and reconstruction by examining basic reconstructed quantities - such as vertex distributions, and to check our neutrino interaction and beam modelling simulation by comparing physics model-dependent quantities such as the PID and total energy distributions. Since the Near Detector data is used directly to predict the Far Detector flux for the oscillation measurement - as will be described later - it is not necessary that the data and simulation perfectly agree for these latter quantities, but it is important to verify that there are no intensity related reconstruction biases between Near Detector data and the simulation, that would not exist in the Far Detector due to the much lower neutrino rate. 
\pend

\vspace{0.1in}
\par

\subsection{Near Detector Distributions}

\pstart
The basic reconstructed quantities, including vertex distributions and track angular distributions are observed to be in good agreement between data and Monte Carlo (as shown in fig~\ref{fig:nd_lowlevel} for events that satisfy the pre-selection cuts).
The distributions of the three PDF distributions that are inputs to the CC/NC PID parameter are shown in figure~\ref{fig:nd_pid} for data and Monte Carlo. In general the shapes of these distributions are well-modelled by the MC. The resulting PID distributions are also shown in figure~\ref{fig:nd_pid} - the shapes of these are also in good agreement - especially in the region $PID>-0.1$, which is used for the flux extrapolation to the Far Detector. The residual shape difference between data and MC below $PID=-0.1$ is used to estimate the uncertainty on the NC contamination in the CC-like sample, as will be described later.
\pend

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{./fig/NDComp_4plots_bw.eps} 
\caption{Distributions of the three input Probability Density Functions to the CC/NC Particle Identification (PID) parameter for Near Detector data and Monte Carlo. The bottom-right plot shows the PID distribution that derives from these three PDFs. 
  } \label{fig:nd_pid} 
\end{figure}


%\begin{figure}[h]
%\centering
%\includegraphics[width=\columnwidth]{./fig/datamcrat_prd.eps} 
%\caption{Near Detector Data/MC spectrum ratios for six beam configurations. The error bars represent statistical errors only.} \label{fig:nd_specrat}
%\end{figure}




\subsection{Far Detector Distributions}
\pstart
We also performed the same checks on the selected sample of Far Detector Data events. A visual scan of the events was carried out in order to ensure that there was no evidence of background contamination in the selected event sample and that the events were well-reconstructed. Figure~\ref{fig:fd_vtx} shows that the reconstructed vertex distributions of the Far Detector events that pass the pre-selection cuts are consistent with the Monte Carlo expectation (the Monte Carlo distributions are normalised to the same number of events as the data to account for the possible effects of oscillations).
\pend

\begin{figure}[h]
\centering

\includegraphics[width=\columnwidth]{./fig/prd_fd_vertices.eps} 

 
\caption{Distributions of track vertices for Far Detector data and Monte Carlo after pre-selection cuts. The Monte Carlo distributions are normalised to the same number of events as the data} \label{fig:fd_vtx} 
\end{figure}


\vspace{0.1in}
\par

\pstart
Figure~\ref{fig:fd_pid} shows the distributions of the three input variables that are used in the charged-current event selection, and the resulting PID parameter itself. Since these variables are sensitive to neutrino oscillations, the Monte Carlo prediction is shown with and without oscillations (where the mixing parameters are chosen to be the best fit values obtained from the fit to the Far Detector reconstructed energy spectrum, described below). The data is well-described by the oscillated Monte Carlo prediction in all of these distributions. 
\pend



\begin{figure}[h]
\centering

\includegraphics[width=\columnwidth]{./fig/prd_fd_pid.eps} 

 
\caption{Distributions of the three input Probability Density Functions to the CC/NC Particle Identification (PID) parameter for Far Detector data and Monte Carlo. The bottom-right plot shows the PID distribution that derives from these three PDFs. The Monte Carlo distributions are shown both without oscillations (solid histograms) and weighted by the best-fit neutrino mixing parameters from the oscillation analysis described below (dashed histograms).
  } \label{fig:fd_pid} 
\end{figure}


\pstart
In conclusion, we have observed a satisfactory level of agreement between basic reconstructed distributions for data and Monte Carlo in both Near and Far detectors - which indicate that no significant reconstruction or intensity-related biases exist in the data. We have observed differences in the shape and overall rate of the reconstructed energy spectra in several beam configurations, which is consistent with known systematic uncertainties in beam flux and cross-section predictions. Since we do not beleve that these differences are due to reconstruction biases, the measured spectum can be used ``as-is'' to predict the Far Detector flux. However, we can use the information contained in the measured Near Detector spectra for the various beam configurations to provide constraints on our beam model, and therefore improve the level of agreement between data and Monte Carlo - the procedure for which will now be described.
\pend




%\subsection{Estimating NC background contamination from ND data}
%\ecom{This section on NC backgrounds breaks up a nice transition between the Data/MC spectra agreement and the description of the tuning procedure. I think we ought to move this later in the paper, nearer to the fitting section.}
%\input{nc_from_alysia_edit.tex}
%      <!-- Local IspellDict: american -->


==> extrapolation.tex <==
%%%%%%%%%%%%%%%%%%%% SYSTEMATICS %%%%%%%%%%%%%%%%%%%%%%


\subsection{Calculation of systematic errors on the predicted FD spectrum}

\pstart
A procedure to identify the most important sources of systematic uncertainty on the measurement of $\dm$ and $\st$ was carried out using fake datasets generated from Monte Carlo. These were produced for both Near and Far detectors and were analysed in the same way as the real data. Each source of systematic error was considered separately and fake datasets were generated with $\pm1\sigma$ shifts of the systematic parameter applied and, in the case of the simulated FD data, oscillations with $\dm=2.72\times10^{-3}$~eV$^{2}$ and $\st=1$. 
\pend

\vspace{0.1in}
\par

\pstart
The systematic error sources considered were the following:
\pend
\begin{itemize}
\pstart
\item Neutral Current Background - estimated uncertainty $\pm50\%$ from a comparison of the shape and normalisation of the observed Near detector data PID distribution to the expectation from Monte Carlo, as described above.
\pend
\pstart
\item Intranuclear Re-scattering - estimated uncertainty of $\pm10\%$ on the absolute shower energy scale, which is based on the change in the visible shower energy spectrum from the Monte Carlo, when the limiting cases of `full pion absorption' and no intranuclear re-scattering are considered.
\pend
\pstart
\item Absolute Normalization - estimated uncertainty of $\pm4\%$, based on uncertainties in fiducial volume uncertainties ($\sim2\%$), relative Near/Far reconstruction efficiencies (estimated from a visual scan of ND and FD data and Monte Carlo - $\sim 2-3\%$)  and POT counting ($\sim 1\%$).% and Monte Carlo POT estimates. 
\pend
\pstart
\item Beam Tuning - The beam tuning procedure described in the previous section applies corrections to the $\xf,\pt$ distributions in the Monte Carlo that result in changes in the $\leten$ visible energy spectrum of $\sim10\%$ around the peak, and $\sim30\%$ in the high energy tail. We have conservatively assigned a $50\%$ error on the magnitude of this correction as an estimate of the uncertainty on the beam tuning procedure. 
\pend
\pstart
\item Charged-current cross-sections - uncertainties of $\pm10\%$ in the axial vector masses for quasi-elastic and resonance production processes are assigned. Uncertainties of $\pm20\%$ are applied to the cross-sections of low-multiplicity DIS events in the Resonance-DIS overlap region. See the previous section on modelling neutrino interactions for details of these error estimates.
\pend
\pstart
\item Shower energy scale calibration - A $\pm6\%$ uncertainty on the absolute shower energy scale is assumed, based on a comparison of test beam measurements in the Calibration detector and the Monte Carlo simulation. Also, a $\pm2\%$ relative uncertainty between Near and Far detectors is assumed, based on uncertainties in calibrating the MINOS detetors using stopping muons.
\pend
\pstart
\item Muon energy scale - assumed $2\%$ relative muon energy scale uncertainty based on studies of fully contained muon tracks recontructed in the Near Detector. The difference between the momentum obtained from the track range and the momentum obtained from a fit to the curvature of the track due to the magnetic field of the detector was examined for both data and MC events, as a function of the range momentum. The deviation of this quantity between data and Monte Carlo was observed to be less than 2\%, which was taken as an estimate of the uncertainty on the magnetic field calibration in the Near Detector, and hence the error on the relative muon energy scale between Near and Far. 
\pend
\pstart
\item CC selection efficiency - applied a shift of $\pm0.02$ in the PID cut that is applied to the fake data samples. This changes both the number of true charged-current and neutral current events that are classified as CC-like. The magnitude of this shift was obtained from a comparison of the data and Monte Carlo PID distributions in the Near Detector. 
\pend
\end{itemize}




\subsubsection{Sensitivity to systematic errors for the different extrapolation methods}


\pstart
The main advantage of the direct extrapolation methods (Beam Matrix and F/N ratio) is that the two largest sources of error on the predicted spectrum, due to 
cross section uncertainties and beam modelling (mainly hadron
production) related uncertainties cancel out when the ND data is used directly to predict the FD spectrum, without the need for prior tuning of the Monte Carlo to better match the measured ND spectrum.  
This is clearly illustrated in figure~\ref{fig2} which shows the extent to which beam and cross-section related uncertainties are reduced using the Beam matrix extrapolation method. Fake datasets were prepared with $\pm1\sigma$ shifts in the beam model (left-hand plot) and cross-section uncertainties (right-hand plot), using the Monte Carlo procedure described above. The black lines in the plot show the ratio of the visible energy spectra of these shifted datasets relative to the nominal Monte Carlo in the Near Detector. These shifted spectra are then used to predict the unoscillated spectra in the Far Detector, and the red histograms show the resulting ratio of the predicted FD spectra to the expected FD spectrum (from the FD fake dataset that is generated with the same systematic shift that is applied to the ND fake dataset). The plot shows that the large initial differences between fake data and Monte Carlo are substantially reduced using this extrapolation technique. 
\pend

\pstart
Figure~\ref{fig:systndfit} shows the same comparison as Figure~\ref{fig2}, but for the NDFit method. The right-hand panel of this plot shows that the NDFit extrapolation is quite successful in reducing the effect of cross-section errors on the extrapolated spectrum. However, the left-hand plot, which is for beam-related uncertainties and does not include a prior beam-tuning step in the extrapolation, shows less complete cancellation of systematic errors than the direct extrapolation methods, and illustrates that Monte Carlo tuning is a much more important component of the fit methods. 
\pend

\pstart
With additional information that will enable us to more cleanly factorise beam and cross-section related uncertainties, the fit methods can potentially provide more powerful constraints on the systematic errors. However, given that our current largest uncertainties on the predicted spectrum are due to beam and cross-section errors, we have decided to use one of the direct extrapolation methods to obtain our primary oscillation result. We chose the Beam Matrix method as our primary extrapolation technique, since it was shown to be more robust to systematic errors that the F/N ratio method, using the fake data MC technique that we outlined above.
\pend
     

\begin{figure}[h]
\centering
\begin{tabular}{cc}

\includegraphics[width=0.45\columnwidth]{./fig/farnear_ratio_beam.eps} 

& \includegraphics[width=0.45\columnwidth]{./fig/farnear_ratio_xsec.eps} \\ 

\end{tabular}
 \caption{Monte Carlo evaluation of the sensitivity of the Beam Matrix method to beam and cross-section related  uncertainties. See accompanying text for details  \label{fig2} }
\end{figure}



\begin{figure}[h]
\centering
\begin{tabular}{cc}

\includegraphics[width=0.45\columnwidth]{./fig/NDFD_SKZP2Par0.eps} 

& \includegraphics[width=0.45\columnwidth]{./fig/NDFD_CCMA.eps} \\ 


\end{tabular}
 \caption{As Figure~\ref{fig2} but for the NDFit extrapolation method. \ecom{The current plot on the left is not exactly ideal, but can serve placeholder figure until a better alternative can be found to illustrate that the fit methods require some form of beam tuning to reduce beam-related systematic errors. Also need to make the line styles for this plot and figure ~\ref{fig2} consistent}} \label{fig:systndfit} 
\end{figure}




\subsubsection{Leading Systematic Uncertainties}
\pstart

As a result of this study, the three largest contributions to the systematic error for the Beam Matrix method were found to be a) the 4\% uncertainty in the overall normalisation; b)  uncertainties in the absolute hadronic energy scale due to intranuclear rescattering, and c) uncertainties in the neutral current background rate. The systematic shifts calculated for the other sources of uncertainty were found to be small in comparison. Table~\ref{tab:oscsyst} shows the magnitudes of the systematic shifts obtained from this procedure. As expected from the above discussion, uncertainties due to beam modelling and cross-sections (entries d) and e) in the table) - which are common to the two detectors - largely cancel out in the extrapolation. The three largest uncertainties (a, b, and c) are included as systematic nuisance parameters in the Far Detector oscillation fit, which is described in the following section. By fitting for these systematic parameters simultaneously using both Near and Far detector data, the effect of these uncertainties are substantially reduced, due to significant cancellations of these errors between Near and Far.  
\pend

\begin{table}[h] 
\begin{center} 
      \begin{tabular}{llcc}
	\hline
	\hline
	Uncertainty &&\dmsq & \sintwo \\
	  && $(10^{-3}\,\mathrm{eV}^2)$ & \\
	\hline
	(a) Normalization & $(\pm 4\%)$          & 0.050 & 0.005\\
	(b) Abs. hadronic E scale & $(\pm 11\%)$ & 0.057 & 0.048\\
	(c) NC contamination &$(\pm 50\%)$       & 0.090 & 0.050\\
	\hline
	(d) Beam uncertainties &    & 0.015 & $<$0.005\\
	(e) Cross sections  &       & 0.011 & 0.005\\
	All other systematics &                  & 0.041 & 0.013\\
	\hline
Statistical Error &   & 0.35 & 0.13\\
        \hline
	\hline
      \end{tabular}
\caption{Systematic shifts on the measurement 
	of \dmsq{} and \sintwo{} for various sources of systematic error, calculated using Monte Carlo generated with the best-fit oscillation parameters obtained from the FD data.
	The values quoted are the average shifts for $\pm$ 1 standard deviation variations in each of the systematic parameters.  
        The last row of the table shows the expected statistical uncertainty on the measurement of \dm and \sintwo for an exposure of $1.27\times 10^{20}$~POT.
	The shifts on \dmsq and \sintwo are treated as uncorrelated, and correlations between the various systematic effects are not taken 
	into account.\label{tab:oscsyst}}
\end{center}  
\end{table}

%      <!-- Local IspellDict: american -->


==> makefile <==
BIBINPUTS=./
prog=latex
mfprog=$(HOME)/texmf/tex/latex/feynmf/feynmf.pl
all: cc_prd.ps cc_prd.pdf

cc_prd.dvi: cc_prd.tex $(shell ls *.tex | grep -v diagrams.tex | grep -v '*diagram.tex')
	$(prog) $<
	bibtex $(shell echo $< | sed 's\.tex\\')
	$(prog) $<
	$(prog) $<
	$(prog) $<


diagrams.dvi: diagrams.tex
	$(mfprog) $<

%_diagram.dvi: %_diagram.tex
#	rm fmftempl.tfm
	$(mfprog) $<

cc_prd_2up: cc_prd.ps
	a2ps -2 --sides=duplex -o cc_prd_2up.ps $<
	ps2pdf cc_prd_2up.ps cc_prd_2up.pdf

%.ps: %.dvi
	dvips $< -o $@
	rm $<

%.eps: %.dvi
	dvips -E $< -o $@
	rm $<


%.pdf: %.ps
	ps2pdf $< $@

